GeoMem-VLA: Internalizing 3D Scene Understanding into Temporal Memory for Vision-Language-Action Models

Vision-Language-Action (VLA) models typically predict actions from current 2D observations, whereas existing 3D policies infer geometry per step without retaining it across an episode. Action generation under occlusion and across multiple stages requires a compact spatial abstraction that persists over time without reconstructing a full 3D scene at each step. Based on this insight, we introduce GeoMem-VLA, a framework that internalizes explicit 3D scene and motion supervision into learnable latent GeoPlantokens, leaving the vision-language backbone's native visual embeddings unaligned. During training, a frozen geometry teacher and demonstration trajectories supervise these tokens via an auxiliary flow-matching head over current scene point maps and future end-effector tracks. Across steps, the policy stores observation and GeoPlan representations in separate memory banks, merges similar adjacent states into event memories, and fuses retrieved history with current features to predict actions. At inference, the 3D teacher and auxiliary head are removed, and action generation relies solely on the latent GeoPlan tokens and episode memory without explicit scene reconstruction. GeoMem-VLA achieves average success rates of 98.9% on LIBERO, 91.10% and 91.24% on RoboTwin 2.0 Clean and Randomized settings, and 78.0% across five real-world manipulation tasks.

==> resources/packages.tex <==
% For flexible citation formats (author-year, numeric)
\usepackage{natbib}

% For UTF-8 encoded CJK (Chinese, Japanese, Korean) characters
\usepackage{CJKutf8}

%\newcommandx
\usepackage{xargs}  

% todo notes
\usepackage{todonotes}  

% multirow
\usepackage{multirow}


% cref
\usepackage{cleveref}

\usepackage{amsmath}
\usepackage{dsfont}

% % using itemize
% \usepackage{enumerate}


\usepackage{subcaption}


\usepackage{svg}

